MVMR: A New Framework for Evaluating Faithfulness of Video Moment Retrieval against Multiple Distractors

With the explosion of multimedia content, video moment retrieval (VMR), which aims to detect a video moment that matches a given text query from a video, has been studied intensively as a critical problem. However, the existing VMR framework evaluates video moment retrieval performance, assuming that a video is given, which may not reveal whether the models exhibit overconfidence in the falsely given video. In this paper, we propose the MVMR (Massive Videos Moment Retrieval for Faithfulness Evaluation) task that aims to retrieve video moments within a massive video set, including multiple distractors, to evaluate the faithfulness of VMR models. For this task, we suggest an automated massive video pool construction framework to categorize negative (distractors) and positive (false-negative) video sets using textual and visual semantic distance verification methods. We extend existing VMR datasets using these methods and newly construct three practical MVMR datasets. To solve the task, we further propose a strong informative sample-weighted learning method, CroCs, which employs two contrastive learning mechanisms: (1) weakly-supervised potential negative learning and (2) cross-directional hard-negative learning. Experimental results on the MVMR datasets reveal that existing VMR models are easily distracted by the misinformation (distractors), whereas our model shows significantly robust performance, demonstrating that CroCs is essential to distinguishing positive moments against distractors. Our code and datasets are publicly available: https://github.com/yny0506/Massive-Videos-Moment-Retrieval.

==> file_sources/fig_dist_em.tex <==
\begin{figure}[!h]
\newcommand\x{3.8}
\newcommand\p{0.48}
\vspace{-.2cm}
\begin{subfigure}[t]{\p\linewidth}
    \centering
    \includegraphics[width=\x cm]{files/em_charades.pdf}
\end{subfigure}
\begin{subfigure}[t]{\p\linewidth}
    \centering
    \includegraphics[width=\x cm]{files/em_anet.pdf}
\end{subfigure}
% \begin{subfigure}[t]{\p\textwidth}
%     \centering
%     \includegraphics[width=\x cm]{files/em_tacos.pdf}
%     \vspace{-0.1cm}
%     \caption{EMScore Distribution}
% \end{subfigure}
\vspace{-.1cm}
\caption{\textbf{EMScore Similarity Distribution.}}
\vspace{-.2cm}
\label{fig:fig_dist_em}
% \vspace{-0.2cm}
\end{figure}



==> file_sources/fig_dist_simcse.tex <==
\begin{figure}[!h]
% \vspace{-.3cm}
\begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=3.8cm]{files/cluster_charades.pdf}
    % \vspace{-0.4cm}
\end{subfigure}
\begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=3.8cm]{files/cluster_anet.pdf}
    % \vspace{-0.4cm}
\end{subfigure}
% \vspace{-.4cm}
\caption{\textbf{SimCSE Similarity Distribution.}}
\vspace{-.1cm}
\label{fig:fig_dist_simcse}
% \vspace{-0.1cm}
\end{figure}



==> file_sources/fig_dist_total.tex <==
\begin{figure*}[!ht]
\newcommand\x{4.4}
\newcommand\p{0.33}

\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/cluster_charades.pdf}
\end{subfigure}
\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/cluster_tacos.pdf}
    \subcaption{SimCSE Distribution}
\end{subfigure}
\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/cluster_anet.pdf}
\end{subfigure}

\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/em_charades.pdf}
\end{subfigure}
\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/em_tacos.pdf}
    \subcaption{EMScore Distribution}
\end{subfigure}
\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/em_anet.pdf}
\end{subfigure}
\caption{\textbf{The Visulization of the SimCSE and EMScore Similarity Distribution.}}
\label{fig:fig_dist_total}
% \vspace{-0.47cm}
\end{figure*}



==> file_sources/fig_examples.tex <==
\begin{figure*}[hbtp]
\newcommand\x{12}
\newcommand\p{0.99}

\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/figure_ex_cha.pdf}
    \vspace{-0.4cm}
\end{subfigure}

\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/figure_ex_anet.pdf}
    \vspace{-0.1cm}
\end{subfigure}

\begin{subfigure}[t]{\p\textwidth}
    \centering
    \includegraphics[width=\x cm]{files/figure_ex_tacos.pdf}
    \vspace{-0.1cm}
\end{subfigure}
\caption{\textbf{Examples of multiple positive moments derived using our methods.} Each query corresponds to that of Charades-STA, ActivityNet, and TACoS, sequentially.}

% \begin{subfigure}[t]{\p\textwidth}
%     \centering
%     \includegraphics[width=\x cm]{files/hist_simcse.pdf}
%     \vspace{-0.1cm}
% \end{subfigure}

\vspace{-.6cm}
\label{fig:fig_ex}
% \vspace{-0.47cm}
\end{figure*}



==> file_sources/fig_human_eval.tex <==
\begin{figure}[!h]
\newcommand\x{15}
\newcommand\p{0.8}
\begin{subfigure}[t]{\p\linewidth}
    \centering
    \includegraphics[width=\p\linewidth]{files/human_eval_sheet.pdf}
    % \vspace{-0.4cm}
\end{subfigure}
\caption{\textbf{Human Evaluation Sheet Example.}}

% \begin{subfigure}[t]{\p\textwidth}
%     \centering
%     \includegraphics[width=\x cm]{files/hist_simcse.pdf}
%     \vspace{-0.1cm}
% \end{subfigure}

% \vspace{-.6cm}
\label{fig:fig_hm}
% \vspace{-0.47cm}
\end{figure}



==> file_sources/fig_simcse_hist.tex <==
\begin{figure}[t]
\centering
\vspace{-0.1cm}
\includegraphics[width=3.8cm]{files/hist_simcse.pdf}
% \vspace{-0.2cm}
\caption{\textbf{Histogram of SimCSE Similarity.}}
\vspace{-0.1cm}
\label{fig:fig_simcse_hist_new}
\end{figure}


% \begin{subfigure}[t]{\p\textwidth}
%     \centering
%     \includegraphics[width=\x cm]{files/cluster_anet.pdf}
% \end{subfigure}


==> file_sources/fig_word_cohesiveness.tex <==
\begin{figure}[!h]
\vspace{-.2cm}
\begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=3.7cm]{files/Charades-STA_word_cohesiveness.pdf}
    % \vspace{-0.4cm}
\end{subfigure}
\begin{subfigure}[t]{0.48\linewidth}
    \centering
    \includegraphics[width=3.7cm]{files/ActivityNet_word_cohesiveness.pdf}
    % \vspace{-0.4cm}
\end{subfigure}
\vspace{-.3cm}
\caption{\textbf{Cohesiveness of the Positive and Negative sets.} The X and Y axes mean the word cohesiveness (word co-occurrence ratio) and its frequency, respectively. The closer the word's co-occurrence ratio approaches 1.0, the more cohesive it is.}
\vspace{-.3cm}
\label{fig:fig_word_cohesiveness}
\end{figure}



==> file_sources/table1_prev.tex <==
\begin{table*}[t]
\centering
\resizebox{1.0\textwidth}{!}
{
\begin{tabular}{@{}clcccccccccccc@{}}
\toprule
Dataset                    & \multicolumn{1}{c}{Model}               & R@1          & R@1           & R@1           & R@5          & R@5           & R@5           & R@20         & R@20          & R@20          & R@50         & R@50         & R@50           \\ 
      &               & IOU0.3          & IOU0.5          & IOU0.7          & IOU0.3          & IOU0.5          & IOU0.7          & IOU0.3          & IOU0.5          & IOU0.7          & IOU0.3          & IOU0.5          & IOU0.7          \\ \midrule
\multirow{5}{*}{$\text{\ourtask}_\text{Charades-STA}$}  & CET & 3.96 & 2.96 (41.77) & 2.02 (21.80) & 15.34 & 11.79 (61.10) & 6.97 (40.91) & 39.85 & 32.21 & 19.91 & 59.58 & 50.54 & 33.88 \\
                           & BET & 4.57 & 2.99 (38.25) & 1.94 (20.73) & 14.26 & 10.98 (61.29) & 7.00 (39.27) & 31.05 & 25.11 & 16.55 & 45.88 & 37.86 & 26.08 \\
                           & G2L & 4.30 & 2.78 (45.50) & 1.97 (25.32) & 14.34 & 10.59 (82.97) & 7.36 (53.18) & 40.89 & 34.74 & 21.33 & 71.92 & 62.72 & 44.82 \\ 
                           & MMN & 13.99 & 12.78 (47.18) & 8.40 (27.47) & 37.86 & 33.29 (83.71) & 22.36 (56.96) & 64.80 & 57.83 & 41.71 & 80.11 & 73.09 & 56.75 \\ \cmidrule{2-14}
                           & CroCs$^{\dagger}$ & \underline{18.38} & \underline{16.31} (47.55) & \underline{10.76} (27.80) & \textbf{43.86} & \textbf{39.05} (83.63) & \underline{26.99} (58.28) & \textbf{69.48} & \textbf{62.89} & \underline{46.39} & \underline{82.88} & \underline{76.08} & \underline{60.28} \\
                           & CroCs & \textbf{19.27} & \textbf{17.38} (48.06) & \textbf{11.44} (27.53) & \underline{43.54} & \underline{39.02} (83.82) & \textbf{27.91} (57.66) & \underline{68.08} & \underline{60.98} & \textbf{46.39} & \textbf{82.99} & \textbf{76.29} & \textbf{60.76} \\ \midrule
                           
\multirow{5}{*}{$\text{\ourtask}_\text{ActivityNet}$} & CET & 1.26 (63.68) & 0.90 (46.52) & 0.56 (27.81) & 2.81 (83.23) & 2.32 (72.84) & 1.75 (58.34) & 5.41 & 4.73 & 3.87 & 8.97 & 8.02 & 6.56         \\
                            & BET & 1.56 (62.82) & 1.16 (44.84) & 0.76 (26.73) & 3.02 (84.97) & 2.55 (74.74) & 2.03 (60.27) & 5.30 & 4.64 & 3.80 & 8.13 & 7.10 & 5.88 \\
                           & G2L & 1.66 (64.21) & 1.32 (49.70) & 0.96 (31.94) & 7.82 (86.88) & 6.43 (79.36) & 4.55 (65.89) & 26.84 & 21.66 & 14.81 & 62.99 & 50.07 & 32.99 \\ 
                           & MMN & 13.82 (64.72) & 10.71 (47.93) & 6.93 (29.16) & 31.54 (87.10) & 25.04 (79.39) & 16.55 (64.68) & 54.79 & 44.50 & 30.62 & 73.08 & 62.09 & \underline{45.76}  \\ \cmidrule{2-14}
                           & CroCs$^{\dagger}$ & \underline{16.46} (63.44) & \underline{12.68} (47.17) & \underline{7.87} (28.64) & \underline{36.03} (86.07) & \underline{28.47} (77.43) & \underline{18.16} (62.06) & \underline{57.91} & \underline{46.52} & \underline{31.12} & \underline{73.82} & \underline{62.12} & 44.89 \\
                           & CroCs & \textbf{20.63} (64.25) & \textbf{15.58} (47.82) & \textbf{9.51} (28.52) & \textbf{44.13} (86.34) & \textbf{34.70} (78.40) & \textbf{22.40} (63.45) & \textbf{67.01} & \textbf{55.58} & \textbf{38.55} & \textbf{79.91} & \textbf{70.02} & \textbf{53.20} \\ \midrule
                           
\multirow{5}{*}{$\text{\ourtask}_\text{TACoS}$}     & CET & 8.95 (37.25) & 5.79 (25.0) & 3.89 & 26.18 (60.25) & 18.88 (46.50) & 12.17 & 54.84 & 42.53 & 23.70 & - & - & - \\
                           & BET & 8.22 (30.37) & 5.30 (18.0) & 2.97 & 29.46 (60.96) & 14.84 (44.61) & 8.32 & 55.67 & 39.76 & 21.51 & - & - & - \\
                           & G2L & 8.72 (39.31) & 5.82 (25.11) & 4.31 & 30.61 (61.47) & 21.51 (46.49) & 12.29 & 56.52 & 42.35 & 22.52 & - & - & - \\ 
                           & MMN & 10.56 (39.20) & 8.61 (26.27) & 5.60 & 36.16 (62.11) & 25.84 (47.42) & 15.47 & 58.20 & 43.89 & 23.80 & - & - & - \\ \cmidrule{2-14}
                           & CroCs$^{\dagger}$ & \textbf{13.43} (38.97) & \underline{10.75} (27.62) & \underline{6.76} & \underline{36.45} (61.51) & \underline{27.01} (47.46) & \underline{15.28} & \underline{58.30} & \underline{44.38} & \textbf{25.16} & - & - & - \\
                           & CroCs & \underline{13.24} (38.44) & \textbf{10.75} (27.39) & \textbf{7.30} & \textbf{39.22} (61.98) & \textbf{29.68} (47.31) & \textbf{16.50} & \textbf{60.05} & \textbf{44.77} & \underline{24.62} & - & - & - \\ \midrule
\end{tabular}
}
% \vspace{-0.2cm}
\caption{
\textbf{Experimental Results on \ourtask~datasets.} Bolded and under-lined results indicate the $1^{st}$ and $2^{nd}$ best performance, respectively.
CroCs$^{\dagger}$ is the model using only weakly-supervised contrastive learning (\S \ref{ssec:false-neg_contrast}).
CroCs uses both of two contrastive learning methods (\S \ref{ssec:false-neg_contrast} and \S\ref{ssec:hard-neg_contrast}).
% The values in parentheses are the results from the \prevtask~task.
We train all the baselines as three trials and report the averaged \ourtask~scores.
% We implement MMN model from scratch and the implemented model exhibits comparable \prevtask~performance to the results reported in the original MMN paper.
}
\vspace{-0.5cm}
\label{table1}
\end{table*}
